Learning Your Way Without Map or Compass: Panoramic Target Driven Visual Navigation

We present a robot navigation system that uses an imitation learning framework to successfully navigate in complex environments. Our framework takes a pre-built 3D scan of a real environment and trains an agent from pre-generated expert trajectories to navigate to any position given a panoramic view of the goal and the current visual input without relying on map, compass, odometry, or relative position of the target at runtime. Our end-to-end trained agent uses RGB and depth (RGBD) information and can handle large environments (up to $1031m^2$) across multiple rooms (up to $40$) and generalizes to unseen targets. We show that when compared to several baselines our method (1) requires fewer training examples and less training time, (2) reaches the goal location with higher accuracy, and (3) produces better solutions with shorter paths for long-range navigation tasks.

==> pages/datageneration.tex <==
\section{Visual Navigation Datasets}
For visual navigation we used two high resolution RGBD maps of homes and offices, Matterport3D and Stanford 2D3DS. For each of the five scenes we tested on we captured 3 high resolution RGBD datasets, one for training an autoencoder, one for training a learned goal checker, and one for training a navigation policy. To get a list of candidate positions we created a high resolution 2D map of the environment (see Figure \ref{fig:house1_map}) which enabled trajectory planning using Dijkstra's algorithm to plan trajectories through each of the environments. We then rendered 10,000 trajectories per environment. This section will discuss the methodology used to generate these datasets as well as characteristics of the data. 

\subsection{Physics Environment}

In order to generate such a large dataset of labeled RGBD images, we used the Gibson~\cite{GIBSON} simulator. Gibson is a state of the art simulator based on PyBullet~\cite{PYBULLET}. In addition to providing dynamics simulation via PyBullet, Gibson offers a custom built pipeline, \emph{Goggles}, that can render highly realistic images from a simulated renderer. Higher realism in images allows us to train on a dataset that is very similar to the real-world, and therefore makes it easier to transfer our learned navigation algorithm to a real-world robot. Figure \ref{fig:title_picture} shows an example of our model being evaluated using Gibson. The left image is a birds-eye rendering of the robot in a 3D map with a trailing history of poses shown in red, while the right images show the Gibson-rendered current view (top) and goal view (bottom). 

% \begin{figure}[h!]
%     \centering {
%         \includegraphics[width=80mm]{imgs/PIC2.PNG}
%     }
%     \caption{An example of a collision-avoiding search path. An overhead view is given on the left, while the two images on the right are the current robot view (on top) and the goal view (on bottom).}\label{fig:overhead_path}
%     \dw{Replace this image with a top down view of the robot entering a room}
    
% \end{figure}

\begin{figure}[h!]
    \centering {
        \includegraphics[width=80mm]{imgs/house1_overlapped.png}
    }
    \caption{2D map of the house1 environment in the Stanford 2D3DS environment. Each pixel is 0.01m x 0.01m. Valid locations, in white, were determined by extracting the floor vertices from the mesh and then later checking for collisions with the clutter labeled vertices in the mesh to blacken potential obstacles. This was generated to enable path planning inside of a ROS framework. Blue positions are candidate locations used to generate autoencoder, policy, and goal checking data as they all could fit the robot inside them. }\label{fig:house1_map}
\end{figure}

\subsection{2D Scene Maps}
We generated 5 maps of the scenes house1, house2, house17 from Matterport3D and area1 and area2 from Stanford2D3DS. Every cell of the map that offered no collision with obstacles was used as a candidate location for navigation and goal image rendering. Each of the maps used a resolution of 1cmx1cm which allowed for a higher number of candidate locations and higher diversity in captured images. We used bounding boxes of dimension $1cm \times 1cm \times 1.6m$ which is the dimension of a pixel by the height of the robotic agent moving through the environment. We then evaluated the collision of a bounding box which was $0.6m \times 0.6m \times 1.6m$ to find collision free positions the robot will fit in. Once we had these positions we were able to calculate expert trajectories.  

\subsection{Autoencoder RGBD Images}
In order to train the autoencoder network we required a dataset of images using candidate locations captured from generating the map. We sampled a collection of $120,000$ positions in the environment because we found diminishing returns if we added more data after that. The dataset was generated individually for each of the five environments resulting in $600,000$ images for the five autoencoders we trained.

To speed up navigation policy and goal checker training, embeddings were pregenerated after the autoencoder training phase. This represented an approximate 64x space savings for loading the dataset into memory and an approximate 10x speedup in training time. While noise can still be added to embeddings before being fed to the policy network in an attempt to increase generalizability and robustness, we found that this was not necessary.

\subsection{Trajectory Dataset} \label{trajectory_dataset}
The goal of this model is to learn a navigation policy that can act on only RGBD sensor input. For the purpose of demonstrating this ability, we chose to implement a navigation planning algorithm that attempts to follow a trajectory planned using Dijkstra's algorithm with a cost map between two poses and avoids collisions. We take a collection of these trajectories and step through each of them. In order for the trajectory to map onto a sequence of commands that our navigation policy will output, we created a Trajectory Discretization algorith. This algorithm steps through each position calculated using Dijkstra's algorithm in the environment $t_i$, the subsequent position $t_{i+1}$, and a position 25 $t_{i+25}$ steps ahead to determine whether to turn the robot left or right and to move forward. The robot will turn left or right whether the position $t_{i+25}$ is turned at an offset greater than $20^{\circ}$ and will output turns in increments of $10^{\circ}$. Forward commands are given if the robot is farther from the next position $t_{i+1}$ than $0.1m$, and if so moves the robot forward in increments of $0.1m$ until under the threshold. We should 25 steps ahead through testing different values to reduce oscillation of robot turning. Using only the next position would result in the robot constantly recalculating its direction and the agent would turn at every step to face a new direction. 

\begin{figure}[h!]
    \removelatexerror
    \begin{algorithm}[H]
    \caption{Trajectory Discretization}\label{alg:nav_gen_pseudocode}
    trajectories $T$ = $\{ pose_{1}, ... , pose_{N} \} $;
    start\_pose = T[0];\\
    goal\_pose = T[0];\\
    angle\_threshold = $20^{\circ}$;\\
    commands = [];\\
    distance\_step = $0.1m$; \\

    \For{$t_i, t_{i+1}, t_{i+25}$ in $T$}
    {
        heading\_direction = $t_i$ - $t_{i+25}$; \\
        current\_robot\_angle = start\_pose.yaw; \\
        \If{current\_robot\_angle - heading\_direction $>$ angle\_threshold}
        {
            command = $LEFT$ if angle\_difference $>$ 0 else $RIGHT$; \\
            commands.append($command$ for every 10 degree difference); \\
            final\_angle = heading\_direction; \\
        }
        
        unit\_pose\_increment = [cos(final\_angle), sign(final\_angle), 0] * distance\_step; \\
        distance\_to\_goal = position\_distance(current\_position, next\_position); \\
        
        \If{distance\_to\_goal $>$ distance\_tolerance}
        {
            commands.append($FORWARD$ for every $distance\_step$ in $distance\_to\_goal$; \\
        }
        
        return commands, poses;\\
            
        
    }
    \end{algorithm}
    
    \caption{An algorithm for converting a sequence of poses from a path planning algorithm into a sequence of discrete commands to be executed by the agent. The values used in this script, such as $distance\_step$ are the same as what were used in the training data. Our method uses a look ahead algorithm to check several steps ahead when picking a correct orientation. We found during testing that the agent would swerve too frequently if we did not use a future position as the correct heading direction. }
\end{figure}


Once we generated these steps, we executed the trajectory in the Gibson simulator environment capturing the RGBD view along every step. This resulted in a large supervised learning dataset of varying trajectory lengths that we could use for training the agent through the environment. The larger the environment, the larger the trajectories were. See Table \ref{table:environment_statistics} for statistics about each of the datasets we generated. Each cell of the table corresponds to the number of training elements captured for each of the environments and datasets we used. The Goal Checker had 9 images captured for every training example, 1 for the current view and 8 for the panoramic goal. The autoencoder and navigation policy had one image captured per position. Overall we had $3,026,827$ images for training.

\begin{table}[h!]
    \centering
    \caption{Training data statistics}
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{ccccc}
        \toprule
        \textbf{Environment} & \textbf{Autoencoder} & \textbf{Goal Checker} & \textbf{$\#$ Trajectories}  & \textbf{Navigation Policy} \\
        \midrule
        area1 & 107668 & 268971 & 2998 & 995720 \\
        area2 & 119532 & 239305 & 2998 & 695515 \\
        house1 & 113780 & 233341 & 5582 & 299612 \\
        house2 & 112095 & & 5599 & 189789 \\
        house17 & 119852 & & 5600 & 846191 \\
        \bottomrule
    \end{tabular}}
    \label{table:environment_statistics}
\end{table}

\subsection{Training / Testing Split for Trajectory Data}
Validation of our navigation policy model was done using a test dataset containing 400 trajectories consisting of varying numbers of commands/images captured from the trajectory execution rendering. Upon every epoch during training for both the autoencoder and policy networks, we evaluated each network using an evaluation dataset of 20\% of our overall dataset for each to make sure the network was still learning. 

The training and test data both contained varied length episodes, ranging from 200 to 300 timesteps per episode. Each timestep corresponds with a single action, which can be a turn in either direction, a forward movement, or a terminus. Each of the three possible movements (left, right, forward) were controlled by discretely moving the robot in a particular direction, which in our configuration of PyBullet produced deterministic results. Figure \ref{fig:policytrainingdata} shows sample trajectories used in the training set. 

\begin{figure*}
    \centering {
        \includegraphics[width=\textwidth]{imgs/space7_c2.png}
    }
    \caption{For area1 in the Stanford2D3DS dataset \cite{stanford2d3ds} we generated 10,000 trajectories and rendered images at each position along those trajectories. This image shows 10 trajectories in the dataset where the large red sphere is the start position and the large green sphere is the final position in each trajectory.} \label{fig:policytrainingdata}
\end{figure*} 

\subsection{Goal checker dataset}
For each of the five environments, we generated $300,000$ training elements for the goal checker. Each of the training elements corresponded to 9 images, 1 for the current view of the robot and 8 for the panoramic goal. $150,000$ of the elements were considered "correct", meaning they were corresponding to a situation where the network should report done for a trajectory. The remaining $150,000$ were marked "incorrect", or that they should be reported as not done along a trajectory. We generated "correct" examples by placing the robot in one of the candidate locations and perturbing the position by 0.1m within a circle around that position and facing the robot in a random orientation. We'd capture the panoramic goal by moving the robot in a circle or in increments $45^{\circ}$. We wanted our policy to work for goal positions within $0.1m$. For the "incorrect" examples we took two positions that we had not captured data for before and put the robot in a random orientation for the "current" view and a panoramic goal at the other location. We made sure that for the "incorrect" examples the two data points were not within 1.0m of each other, so as to not confuse the network. All of these captured images were then embedded using the autoencoder trained for that environment and stored for training. 

